Integrability of Limit Shapes of the Six Vertex Model

The main result of this paper is the construction of infinitely many conserved quantities (corresponding to commuting transfer-matrices) for the limit shape equation for the 6-vertex model on a cylinder. This suggests that the limit shape equation is an integrable PDE with gradient constraints. At the free fermionic point this equation becomes the complex Burgers equation.

==> sigmafigures.tex <==
\begin{figure}[h]\label{sigmafigures}
\includegraphics[scale=.25]{sigma1} \;
\includegraphics[scale=.25]{sigma2} \;
\includegraphics[scale=.25]{sigma3}
\caption{For this graphic, I chose some function with the right singularities and plotted it.}
\end{figure}
